Inclusive Study Group Formation At Scale

Underrepresented students face many significant challenges in their education. In particular, they often have a harder time than their peers from majority groups in building long-term high-quality study groups. This challenge is exacerbated in remote-learning scenarios, where students are unable to meet face-to-face and must rely on pre-existing networks for social support. We present a scalable system that removes structural obstacles faced by underrepresented students and supports all students in building inclusive and flexible study groups. One of our main goals is to make the traditionally informal and unstructured process of finding study groups for homework more equitable by providing a uniform but lightweight structure. We aim to provide students from underrepresented groups an experience that is similar in quality to that of students from majority groups. Our process is unique in that it allows students the opportunity to request group reassignments during the semester if they wish. Unlike other collaboration tools our system is not mandatory and does not use peer-evaluation. We trialed our approach in a 1000+ student introductory Engineering and Computer Science course that was conducted entirely online during the COVID-19 pandemic. We find that students from underrepresented backgrounds were more likely to ask for group-matching support compared to students from majority groups. At the same time, underrepresented students that we matched into study groups had group experiences that were comparable to students we matched from majority groups. B-range students in high-comfort and high-quality groups had improved learning outcomes.

==> SIGCSE 2023 arXiv Submission/figs_code/boxplots_race.tex <==
\begin{figure}[h]
    \centering
    \includegraphics{figs/race_dem_errorbars.png}
    \caption{Comparisons, between students identifying with differing races, in percentages ($y$-axis) answering positively to key study group quality questions. Students of mixed race were counted multiple times, in each of the racial categories they indicated they identified with. }
    \label{fig:race_boxplots}
\end{figure}

==> SIGCSE 2023 arXiv Submission/figs_code/boxplots_year.tex <==
\begin{figure}[h]
    \centering
    \includegraphics{figs/year_dem_errorbars.png}
    \caption{Comparisons, between students of differing years in undergraduate study, in percentages ($y$-axis) answering positively to key study group quality questions. }
    \label{fig:year_boxplots}
\end{figure}

==> SIGCSE 2023 arXiv Submission/figs_code/demographic_boxplots.tex <==
\begin{figure*}
    \centering
    \includegraphics{figs/gender_dem.png}
    \includegraphics{figs/race_dem.png}
    \includegraphics{figs/year_dem.png}
    \caption{Comparisons between students of differing demographics, in percentages ($y$-axis) answering positively to key study group quality questions, and counts (displayed on bars) answering positively to key study group quality questions. For student race, students of mixed race were counted in each of the racial categories they indicated they identified with. }
    \label{fig:dem_boxplots}
\end{figure*}

==> SIGCSE 2023 arXiv Submission/figs_code/img_matching_flowchart.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/flowchart.pdf}
    \caption{
        \label{fig:flowchart}
        Group matching process flowchart along with a detailed software diagram (in gray). First, students are routed based on whether they want a study group and whether they already have a self-matched group in mind. For the remainder of students, our software uses the student preferences to match them into groups. The algorithm first partitions students based on the most important criteria, forms groups within subdivisions to maximize matches on secondary criteria, and finally then performs checks on the demographic and preference-based breakdown within each group. After ensuring that no singletons are present and performing additional verification, the resulting groups are finalized and displayed.
    }
\end{figure}

==> SIGCSE 2023 arXiv Submission/figs_code/img_matching_timeline.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/timeline.pdf}
    \caption{
        \label{fig:timeline} The timeline of the group assignment process, from initial surveys to the final evaluation, in the context of the homeworks and exams in the class.}
\end{figure*}

==> SIGCSE 2023 arXiv Submission/figs_code/partition_tree_example.tex <==
\begin{figure}
\begin{center}
    \begin{tikzpicture}[->, level distance=1.4cm, sibling distance = 1.4cm, thick, scale=0.8, transform shape]
     
        \node[draw, circle, fill=darkblue!25]{All}  
        child {node [draw, circle, fill=red!25]{Pacific} 
            child { node [draw, circle, fill=darkgreen!50]{Mo} }
            child { node [draw, circle, fill=darkgreen!50]{Tu} }
            child { node [draw, circle, fill=darkgreen!50]{We} }
            child { node {...} }
            %child { node [draw, circle, fill=darkgreen!50]{Th} }
            %child { node [draw, circle, fill=darkgreen!50]{Fri} }
            %child [missing]
            child [missing]
            child [missing]
        }
        child {node [draw, circle, fill=red!25]{Eastern}
            child [missing]
            %child [missing]
            child { node [draw, circle, fill=darkgreen!50]{Mo} }
            %child { node [draw, circle, fill=darkgreen!50]{Tu} }
            child { node {...} }
            %child [missing]
            %child [missing]
        }
        child {node [draw, circle, fill=red!25]{Europe}
            child [missing]
            child [missing]
            child { node[draw, circle, fill=darkgreen!50] {Mo} }
            child { node {...} }
        }
        child {node [draw, circle, fill=red!25]{$\ldots$}
            child [missing]
            child [missing]
            child { node[draw, circle, fill=darkgreen!50] {$\ldots$} }
        };
        
        \node[draw=none, darkblue] at (-4, 0) {\textbf{[All Students]}};
        \draw[->, darkblue] (-2.8, 0) -- (-0.8,0);
        \node[draw=none, red!70] at (-4, -0.7) {\textbf{[Timezone Partitions]}};
        \draw[->, red!70] (-4, -0.9) -- (-2.8,-1.2);
        \node[draw=none, darkgreen] at (-5.2, -1.6) {\textbf{[Scheduling Partitions]}};
        \draw[->, darkgreen] (-5, -1.8) -- (-5,-2.2);
    \end{tikzpicture}
    \caption{\label{fig:multi-partition_tree}An example of class partitions modeled in a tree-like figure. If a student \textit{could} be part of multiple partitions, they are initially placed into \textit{all of these partitions}, which are later pruned to ensure that each student is part of one group. }
\end{center}
\vspace{-5mm}
\end{figure}

==> SIGCSE 2023 arXiv Submission/figs_code/positive_response_correlation_matrix.tex <==
\begin{figure}
    \centering
    \includegraphics{figs/indicator_corrs.png}
    \caption{Pearson correlation matrix of positive responses to study group quality indicators.}
    \label{fig:indicator_corrs}
\end{figure}

==> SIGCSE 2023 arXiv Submission/figs_code/table_demographic_distribution.tex <==
\begin{figure}
    \centering
    \begin{tabular}{|l|llll|}
        \hline
        \textbf{Demographic group} & \textbf{(A)} & \textbf{(B)} & \textbf{(C)} & \textbf{(D)}              \\ \hline \hline
        Women             & 139 & 103 & 74.1\%  &(66.8\%, 81.4\%)      \\ \hline
        Men               & 326 & 221 & 67.8\%  &(62.7\%, 72.9\%)      \\ \hline
        \begin{tabular}[c]{@{}l@{}}Gender non-conforming/\\ Genderqueer \end{tabular} & 2   & 2   & 100\% & - \\ \hline
        Other/Prefer not to answer & 10   & 10   & 100\% & - \\ \hline \hline
        \begin{tabular}[c]{@{}l@{}}Black/ African American\end{tabular}                           & 7  & 6  & 85.7\% & (59.8\%, 100\%)  \\ \hline
        Hispanic          & 39  & 28  & 71.8\% & (57.7\%, 85.9\%) \\ \hline
        \begin{tabular}[c]{@{}l@{}}Native American/ \\Alaska Native/\\ Hawaiian Native \end{tabular} & 9  & 6  & 66.7\% & (35.9\%, 97.5\%) \\ \hline
        White             & 86  & 66  & 76.7\% & (67.8\%, 85.7\%) \\ \hline
        Asian             & 345 & 233 & 67.5\% & (62.6\%, 72.4\%) \\\hline
        Other/Prefer not to answer & 27 & 20 & 74.1\% & (57.5\%, 90.6\%) \\ \hline \hline
        Freshman          & 323 & 214 & 66.2\% & (61.1\%, 71.4\%) \\ \hline
        \begin{tabular}[c]{@{}l@{}}Junior or \\ Senior Transfer\end{tabular}                        & 66 & 53 & 80.3\% & (70.7\%, 89.9\%) \\ \hline
    \end{tabular}
    \vspace{-2mm}
    \caption{Demographic distribution of students in our sample. Column (A): total counts across demographic groups, Column (B): counts across software-matched groups, Column (C): percentage of students within subgroup who requested software-assigned study groups, Column (D): population-level confidence intervals on percentages in column (C).}
    
    \label{fig:self_form_comp}
    \vspace{-4mm}
\end{figure}

==> SIGCSE 2023 arXiv Submission/figs_code/table_grade_assocation_confidence_intervals.tex <==
\begin{figure*}

\centering
\begin{tabular}{llllll}
  \textbf{Student group} &
  {\begin{tabular}[c]{@{}l@{}}\textbf{Indicated positive response to question} \\ \textbf{/ did not indicate positive response}\end{tabular}}  &
  {\begin{tabular}[c]{@{}l@{}} \textbf{MT1 Score} \\ \textbf{(Max 50)} \end{tabular}} &
  {\begin{tabular}[c]{@{}l@{}} \textbf{MT2 Score} \\ \textbf{(Max 50)} \end{tabular}} &
  {\begin{tabular}[c]{@{}l@{}} \textbf{Final Score} \\ \textbf{(Max 100)} \end{tabular}} &
  \textbf{Misc. diff} \\ \mytoprule
\multicolumn{1}{|l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{All software-matched} \\ \textbf{students}\end{tabular}}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Did not request reassignment\\ / did request reassignment 1-3 times\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.27 / 37.71 \\ ( p=0.003)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.72 / 36.42 \\ (p=0.025)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.01 / 67.35 \\ (p=0.046)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable asking questions \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.68 / 36.22 \\ (p=0.022)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.22 / 66.08 \\ (p=0.011)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable sharing ideas \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.04 / 37.60 \\ (p=0.011)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.81 / 35.27 \\ (p=0.002)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}71.96 / 65.86 \\ (p=0.046)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \mytoprule
\multicolumn{1}{|l|}{\textbf{Freshmen}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Did not request reassignment\\ / did request reassignment 1-3 times\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}41.40 / 37.60 \\ (p=0.0006)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.44 / 37.17 \\ (p=0.007)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}74.56 / 68.55 \\ (p=0.046)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable sharing ideas \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.96 / 37.41 \\ (p=0.009)\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} \\ \mytoprule
\multicolumn{1}{|l|}{\textbf{Transfer}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Would take future courses with group \\ / would not\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}32.00 / 39.57 \\ (p=0.001)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}61.02 / 73.71 \\ (p=0.012)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}MT1-MT2: \\ -0.075 / 0.012 \\ (p=0.018)\end{tabular}} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Any group interaction \\ / no interactions with group\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}34.96 / 39.43 \\ (p=0.013)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}32.45 / 38.98 \\ (p=0.005\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}61.65 / 72.81 \\ (p=0.030)\end{tabular}} &
  \multicolumn{1}{l|}{} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Some to most members participated \\ / no members participated\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}35.64 / 39.31 \\ (p=0.024)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}} 33.08 / 39.16 \\ (p=0.009)\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} \\ \mytoprule
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Students receiving a} \\ \textbf{B-, B, B+ on MT1}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Any group interaction \\ / no interactions with group\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.71 / 65.78 \\ (p=0.008)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}MT1-Final: \\ -0.075 / -0.14 \\ (p=0.003)\end{tabular}} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Some to most members participated \\ / no members participated\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}-0.084 / -0.130 \\ (p=0.047)\end{tabular}} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable asking questions \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.99 / 36.53 \\ (p=0.044)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.18 / 63.91 \\ (p=0.004)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}-0.082 / -0.154 \\ (p=0.004)\end{tabular}} \\ \mytoprule
\end{tabular}
\caption{
        \label{fig:ttest_groups}
        Student's t-tests on difference in sample means, between exam grades within demographic groups, split on positive/negative responses to group experience indicators in the group survey. Only cells with significant differences in sample means are highlighted, with p-values provided. The Miscellaneous Differences column contains percentage-score changes for a student group, either from Midterm 1 to the Final, or from Midterm 2 to the Final, as indicated. Final scores were overall lower than midterm scores, so lower decreases in percent scores are interpreted as positive results.  
    }
\end{figure*}

==> SIGCSE 2023 arXiv Submission/figs_code/table_positive_response_students.tex <==
\newcommand{\mytoprule}{\specialrule{0.15em}{0em}{0em}}
\begin{figure}
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Group Quality Indicator} & \textbf{Software-Assigned} & \textbf{Self-Formed} \\
    \mytoprule
    Future courses                                                     & \begin{tabular}[c]{@{}l@{}}52.4\%\\ (47.0\%, 57.8\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}97.2\%\\ (94.5\%, 99.9\%)\end{tabular} \\ \hline
    Group interaction                                              & \begin{tabular}[c]{@{}l@{}}56.6\%\\ (51.3\%, 61.9\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}95.8\%\\ (92.5\%, 99.1\%)\end{tabular} \\ \hline
     Group participation                                                     & \begin{tabular}[c]{@{}l@{}}62.3\%\\ (57.1\%, 67.5\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}95.1\%\\ (91.6\%, 98.6\%)\end{tabular} \\ \hline
    Comfort asking questions                                           & \begin{tabular}[c]{@{}l@{}}74.2\%\\ (69.6\%, 78.9\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}93.7\%\\ (89.7\%, 97.7\%)\end{tabular} \\ \hline
    Comfort sharing ideas                                              & \begin{tabular}[c]{@{}l@{}}78.4\%\\ (74.0\%, 82.9\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}95.1\%\\ (91.7\%, 98.6\%)\end{tabular} \\ \hline
    \end{tabular}
    \caption{ Percentages (with confidence intervals) of students who reported positive responses to the five group quality indicators. First column: Students in software-matched groups. Second Column: Students in self-formed groups.}
    \label{fig:overall_props}
\end{figure}

==> SIGCSE 2023 arXiv Submission/sections/analysis.tex <==
\vspace{-4mm}
\section{Analysis and Evaluation}
\label{sec:evaluation}
\newcommand{\placeholderfig}[1]{{\color{red} PLACEHOLDER FIG TITLE: #1}}

Our analysis is based on responses to the student preference survey, reassignment requests, the final evaluation survey, and grade information. We only consider the 477 students who consented to participate in this research, though many more students participated in the group matching process. 

We consider each of the five questions on the evaluation survey (Sec.~\ref{sec:evalsurvey}) as a group-quality indicator, and we classify positive responses as below:
%We classify a response as powe classify “positive” responses, i.e. indicators that the student had a good experience in their study group, as follows:
\begin{enumerate}
\item Comfort asking questions: Students agreed or strongly agreed that they feel comfortable asking questions in the group
    \item Comfort sharing ideas: Students agreed or strongly agreed that they feel comfortable sharing ideas in the group
    \item Interaction frequency: students interacted with their group at least once a week 
    \item Participation: Some, most, or all members participated% in group interactions
      \item Future courses: students state they hope they can, or definitely will, take future courses with their group
    
\end{enumerate}
% \emph{Statistical tests.}
% We use different statistical tests to determine significance based on the sample size. If the sample sizes in consideration are greater than 30, we use a 2-sample proportion z-test with $\alpha = 0.05$ (referred to as a z-test in the remainder of the text), else we use a Fisher exact test ($\alpha = 0.05$) for small sample sizes~\cite{rice2006mathematical}.



\subsection{Participation demographics} \label{sec:partdemo}
\input{figs_code/table_demographic_distribution}
Fig.~\ref{fig:self_form_comp} showcases different demographic breakdowns of our participants, as well as breakdowns across those who chose self-matched vs. software-matched groups. 
143 students reported having self-matched groups and 334 students asked for software-matched groups. %self-matched groups reported extremely positive results across all the metrics, as can be observed in the rightmost column of Fig.~\ref{fig:overall_props}. One perspective is that self-matched groups can be viewed as a gold standard, where students already know they feel comfortable and productive when working with students they choose.
Looking at the percentages in of students who requested software-matched groups in Column (C) in Fig.~\ref{fig:self_form_comp}, we see that women and gender-nonconforming/ genderqueer students were more likely to request software-matched study groups than men, and Black, Hispanic and White students were more likely to request software-matched groups than Asian students (the largest demographic group).  



\emph{Requesting reassignments.} 
27\% of students requested one reassignment and 2\% of students requested two reassignments. 
Significantly fewer Asian students requested reassignment (24\%) compared to non-Asian and non-White students (39\%). Hispanic students (48\%) (and White students (41\%)) requested reassignments significantly more often than non-Hispanic (28\%) (non-White (26\%)) students, respectively, indicating that initial group matches did not work out as well for these students. Significance in all these cases was verified using 2-sample proportion z-tests, $\alpha = 0.05$~\cite{rice2006mathematical}.

\emph{Software-matched students.}
Software-matched students had overall positive group experiences. For example, 74\% and 78\% of students reported feeling comfortable asking questions and sharing ideas respectively. We performed significance tests in comparison to the null hypothesis that 50\% of students would have positive study group experiences and 50\% of students would have negative study group experiences. Using a 2-sample proportion z-test ($\alpha=0.05$)~\cite{rice2006mathematical}, over 50\% of all software-matched students had positive experiences with group interaction, group activity, and comfort asking questions and sharing ideas. %, as can be noted in the second column of Fig.~\ref{fig:overall_props}. 


We note that positive responses to the evaluation questions tended to correlate with each other, using the Pearson correlation coefficient. Specifically, positive responses to the group interaction and group participation questions were correlated with each other ($r = 0.83$) . Additionally, the comfort indicators correlated with each other ($r = 0.79$). 


\emph{Self-matched students.} We find that self-matched students had even more positive experiences than software-matched students (93\% and 95\% report comfort in asking questions and sharing ideas respectively), similar to the findings of~\cite{lovold2020forming}. This is not surprising since many of the self-matched groups are formed by students who knew each other before college. The remaining analysis focuses on software-matched students.



%We notice that students of underrepresented demographics were more likely than majority students to request study groups. For example we observe, in the second section of column C of Fig.~\ref{fig:self_form_comp}, that  Similarly, proportions of women and gender non-conforming / genderqueer students requesting software-matched study groups are higher than proportions of men, observable in the first three rows of Fig.~\ref{fig:self_form_comp}. Therefore, even though self-matched groups seem to have more positive responses than software-matched groups, it is useful to a large population of students, and especially traditionally underrepresented students, to provide inclusive study group options.





\subsection{Impact on underrepresented students}
%\input{figs_code/demographic_boxplots}
In general, students in software-matched groups who identify as being from an underrepresented racial or gender demographic did not demonstrate significant differences in responses compared to majority demographic groups, with a few exceptions.  

\begin{figure}[h]
    \centering
    \includegraphics{figs/gender_dem_errorbars.png}
    \caption{Responses by gender for three representative questions from the evaluation survey (software-matched students). The percentage of positive responses is on the $Y$-axis, the black bar is an error bar.}%Comparisons, between students identifying as male and female, in percentages ($y$-axis) answering positively to key study group quality questions. }
    \label{fig:gender_boxplots}
    \vspace{-3mm}
\end{figure}

\subsubsection{Gender}
Figure~\ref{fig:gender_boxplots} shows responses to representative survey questions for different gender groups. Each vertical bar corresponds to the percentage of positive responses to the question for a particular gender. Bars that are roughly the same height indicate similar experiences across gender groups. 

Using 2-sample proportion z-tests ($\alpha = 0.05$)~\cite{rice2006mathematical}, we found no significant difference between students in the majority group (men) and those who identified as any other gender (Fig.~\ref{fig:gender_boxplots}). %Additionally, confidently more than half of all women and men students in software-matched groups responded positively to 4 of 5 group quality indicators, aligned with our general population results (see plots 2-5 of group quality indicators in the student gender section, in Fig.~\ref{fig:dem_boxplots}). 

%the yellow (men) and green (women) bars are of similar heights in Fig.~\ref{fig:gender_boxplots}
One student identifying as gender non-conforming / genderqueer (GNC) had positive experiences in all categories, and one other GNC-identifying student had negative experiences in all categories, but the small sample size  prevents any generalizable conclusions.% Due to the very small count of GNC-identifying students, we are not able to generalize these results.

\begin{figure}[h]
    \centering
    \includegraphics{figs/race_dem_errorbars.png}
    \caption{Responses by race for the same questions for software-matched students. %The percentage of positive responses is on the $Y$-axis, the black bar is an error bar. Students identifying with multiple racial groups are counted in each group. 
    Black/AA (green bar) and Hispanic (orange bar) students respond similarly to other groups. }%Comparisons, between students identifying as male and female, in percentages ($y$-axis) answering positively to key study group quality questions. }
    \label{fig:race_boxplots}
    \vspace{-2mm}
\end{figure}


%\input{figs_code/boxplots_race}

\subsubsection{Race}
In this analysis students who self-identified with multiple racial groups are counted in each of the categories.
Fig.~\ref{fig:race_boxplots} shows responses to representative survey questions for different racial groups, in a similar style to Fig.~\ref{fig:gender_boxplots}, for software-matched students. %Each vertical bar corresponds to the responses to a given question for a particular group. Bars that are roughly the same height indicate similar experiences reported across groups. 
We see that students identifying as Black / African-American (AA) did not show statistically significant differences  in any study group indicators, in comparison to non-Black/AA students (using a Fisher exact test, $\alpha =0.05$, since the sample sizes are small~\cite{rice2006mathematical}). All six Black/AA students in the class reported positive indicators.

Similarly, Hispanic\footnote{We recognize that Hispanic is an ethnicity, and not a racial group, per the US Census Bureau, however we include it here to accurately reflect our survey.}-identifying students did not show statistically significant differences from non-Hispanic students (Fisher exact test, $\alpha =0.05$~\cite{rice2006mathematical}). One interesting observation is that even though White students reported similar comfort levels to non-White students, they were significantly less likely than others to want to take courses with their groups again (2-sample proportion z-test, $\alpha=0.05$~\cite{rice2006mathematical}) (Fig.~\ref{fig:race_boxplots}, subfigure 3), which requires further investigation, especially given that White and Hispanic students requested reassignments significantly more often (see Sec.~\ref{sec:partdemo} ). We were unable to make general conclusions about the experiences of students identifying as Native American, Alaska Native, or Native Hawaiian due to the small sample size and mixed responses. 

%wanting to take courses with their study groups less often, number of students who participated in their groups 

%For the six Black/AA students who participated in software-matched study groups, there were very positive experiences across all indicators. 

%Within differing racial subgroups, we find some slight differences in student group experiences. All statistical significance tests for smaller subgroups (Hispanic, Black, and Native American / Alaska Native / Native Hawaiian students) were conducted using the Fisher exact test, and for larger subgroups they were conducted using 2-sample proportion z-tests. Most notably, no significant differences were found between all students of majority racial groups (White or Asian) and all students of underrepresented racial groups (non-White and non-Asian) --- all analyses below on individual racial subgroups support this finding.

%\textbf{Hispanic-identifying students} did not have statistically significant differences in their responses, indicating that final group assignments were comparable in quality to other demographic subgroups. We also note that we can say with 95\% confidence that the majority of Hispanic students felt comfortable asking questions and sharing ideas in their final groups. These findings can be observed in the second row of Fig.~\ref{fig:dem_boxplots}, when qualitatively comparing the height of the percentage bars of Hispanic students to other subgroup bars.

%\textbf{Students identifying as Black / African-American (AA)} did not show statistically significant differences in any study group indicators, in comparison to non-Black/AA students. For the six Black/AA students who participated in software-matched study groups, there were very positive experiences across all indicators. All six students felt comfortable asking questions, and five of six felt comfortable sharing ideas in their groups (Fig.~\ref{fig:dem_boxplots}). The small sample size limits our interpretations here, but this is promising. 

%\textbf{Students identifying as Native American, Alaska Native, or Native Hawaiian} (referred to shorthand as Native), we observed four of the six students indicating positive responses across all study group indicators, and five of the six feeling comfortable asking questions and sharing ideas in their groups (Fig.~\ref{fig:dem_boxplots}). Again, due to small sample sizes, generalizing statements about their experiences or comparisons to other groups cannot be made with confidence. 

%\textbf{White-identifying students} had significantly less positive study group experiences than non-White students in a few categories, namely: wanting to take courses with their study groups less often, number of students who participated in their groups (seen in the second section of Fig.~\ref{fig:dem_boxplots}). 

%\textbf{Asian-identifying students} had significantly more positive study group experiences than non-Asian students (Fig.~\ref{fig:dem_boxplots}). However, when performing tests of significant difference between Asian students and all other non-White or non-Asian students, we found no significant differences in study group quality. Similarly, we found no significant differences in study group experiences between White students and all other non-White and non-Asian students. This may indicate that there are different social and cultural experiences in study groups between two demographics that may be considered majority groups in engineering classrooms at UC Berkeley, but non-majority groups do not face disproportionately different study group experiences in comparison to either. 






%\input{figs_code/table_positive_response_students}








%\input{figs_code/boxplots_year}


\subsubsection{Student year}
Freshmen students had overwhelmingly positive study group experiences (Fig.~\ref{fig:year_boxplots}), with significantly higher proportions of positive responses to all study group indicators in comparison to non-freshmen (2-sample proportion z-test,  $\alpha=0.05$~\cite{rice2006mathematical}). This may because freshmen were more enthusiastic overall, and the course is targeted to freshmen.

\begin{figure}[h]
    \centering
    \includegraphics{figs/year_dem_errorbars.png}
    \caption{Responses by year for the three representative questions for software-matched students. Freshmen students respond significantly more positively for all questions.} %We believe this may because Freshmen were more enthusiastic overall, and the course is targeted to freshmen.}%Comparisons, between students identifying as male and female, in percentages ($y$-axis) answering positively to key study group quality questions. }
    \label{fig:year_boxplots}
    \vspace{-3mm}
\end{figure}


%When considering a student’s year in school at the time of the course, it became clear there are extremely different study group outcomes depending on a student’s year. In many ways, our group matching software was geared towards first-year students, who are the least connected socially. As such, it is promising to note that Freshman students had overwhelmingly positive study group experiences, with significantly higher proportions of positive responses to all five study group indicators in comparison to non-freshmen (Fig.~\ref{fig:dem_boxplots}). 

%Transfer students, however, had significantly less positive responses in the indicators of: group group interaction, group activity, and comfort sharing ideas in their group (Fig.~\ref{fig:dem_boxplots}). This is an additional possible indicator that post-processing matching to ensure non-singletons of certain groups may actually be quite important, our software matcher in Fall 2020 did not fully ensure against student year singletons\footnote{Later iterations of our software allow this.}.  Although we partition on student year to ensure groups predominantly comprised of the same year, transfer students may need to be considered an underrepresented group in themselves, and other as of yet unaddressed factors may impact their study group success.



\subsection{Exam performance}
\label{section:grades_assoc}

%\input{figs_code/table_grade_assocation_confidence_intervals}

We find that just participation in a study group, whether self-matched or software-matched, did not correlate with higher exam scores for students. It makes sense that the specific experiences in the group matter. We consider a student to be in a \emph{high-comfort} study groups if they responded positively to at least one of indicators 1 or 2, and \emph{high-activity} study groups as those where students response positively to at least one of indicators 3 or 4~(using indicators defined at the beginning of Sec.~\ref{sec:evaluation}). 

We identify several correlations with software-matched high-comfort and high-activity groups. Students in high-comfort groups had higher final exam scores (average = 72.2\%) than others (average = 66.1\%) (p = 0.011, Student's t-test~\cite{rice2006mathematical}). We examined more closely student performance in different grade ranges. 
 Students with B-range scores (68-89\%) on the first midterm (we call these B-range students) who were also in high-comfort groups saw significantly higher final exam grades than B-range students not in high-comfort groups (72.2 \% vs. 63.9\%, p = 0.004, Student's t-test~\cite{rice2006mathematical}). Similar gains were also observed on the final exam for B-range students in high-activity groups vs. those not in high-activity groups (71.7\% vs. 65.8\%, p=0.008, Student's t-test~\cite{rice2006mathematical}). Students who received A, and C to below C-level, grades on MT1 had no significant associations between their scores and group quality indicators. %This suggests that for students who entered 
 
 %We also examined the difference between the MT1 performance and the Final performance: B-range students in high-comfort (high-activity) groups decreased their score by only $0.08$ ($0.075$), 
 
% Additionally, knowing that the general distribution of Final scores was much lower than MT1 scores, students at the B-range in both high-comfort and high-activity groups demonstrated significantly lower decreases from MT1 to the Final.
 
\subsection{Study-group obstacles}
34.5\% of students reported no major obstacles in their study groups. Despite the fact that our matching system explicitly prioritized student availability, students struggled to schedule group meetings, and 48.5\% of students reported this as a challenge they faced. Over 31.7\% reported that Zoom fatigue obstructed the success of their meetings and 30.7\% also found interactions with students they did not know awkward. Of students listing other reasons, multiple students indicated that lack of responsiveness from their group mates was a challenge in establishing the study group. 
 
 %associated with several factors: frequently interacting groups, multiple group members participating, and feeling comfortable asking questions in their groups (Fig.~\ref{fig:ttest_groups}). 

% 
 
 
%At the classroom-level, all software-matched students demonstrated significant associations between feeling comfortable sharing ideas in their groups, and increases in both midterm and final exam scores, as seen in the top section of Fig.~\ref{fig:ttest_groups}. For example, in the "Final score" column of the second row in  Fig.~\ref{fig:ttest_groups}, we observe that students who felt comfortable asking questions averaged 72.22 on the final, versus students who didn't feel comfortable asking questions averaging near 66.08, with a confidence of 98.9\% of the first score being higher. Similar results were seen around comfort sharing ideas, as well as not requesting reassignments. All software-matched students also demonstrated significant associations between feeling comfortable sharing ideas in their groups, and increases in Midterm 2 (MT2) and Final scores. 


\section{Limitations}
%Our conclusions are limited by a few factors. 
Unfortunately, we are limited in generalized conclusions due to the small sample sizes of some of the demographic groups, which is the reality of many CS courses. Informal anecdotal feedback from students in underrepresented groups was positive, and we plan to conduct formal focus groups in the future. 
% to better understand this. % and much of it was positive, this was not done formally. 
Our setting makes it difficult to run a randomized control study, since it would be unethical to disallow students from joining a study group. % who wanted a study group from joining one. %Hence our conclusions are correlation-based, and we cannot say anything about causation. 
%We are also unable to run a truly randomized control study, since we do not want to prevent a student who wants a study group from joining one. Our conclusions are only correlation-based, and it is difficult to draw causation. 
%Since the study groups were opt-in, we do not have any randomized control data, and since we do not want to ever prevent a student who wants a study group from having one, it will be difficult to conduct a truly randomized experiment ever. 
The experiment was conducted during a remote semester, and further work will be required to explore how these conclusions hold in the context of in-person instruction. The PI for the study was also the instructor for the course, and strongly encouraged group participation, which may have increased participation. % It is possible that fewer students would participate in absence of this encouragement. It is also possible that students who had positive experiences were more likely to consent to the research study, and thus our data may be biased. 
There are multiple sub-optimalities in the implementation of our partitioning algorithm. In particular, the process of merging small partitions together could be optimized based on partition size. Partnering to avoid solo-status could be done before group formation as well. We can also optimize the random assignment in large partitions. %We intend to work on improving these for better group outcomes, as well as incorporate established algorithms from the literature.  

% groups are randomly assigned in large partitions, and we hope to improve on this in the future. %Additionally, we hope to explore different approaches for partnering students in avoiding solo-statu
%The algorithm can lead to uneven partitions, some may have large numbers of students (e.g. those corresponding to popular study times) and others may have much lower numbers of students. The current approach does optimize matches in large partitions, which we hope to improve in future work.
%Asian is too broad a category. 
\vspace{-2mm}
\section{Discussion}
This work provides an example of how a structured approach to study group formation can provide similar experiences for students from different demographic groups. This system is clearly filling an unmet need for underrepresented students, given the differential rates at which Black, Hispanic and women students requested study groups as compared to their peers. %Students who are more connected in the social network (e.g. those coming from feeder schools) are more easily able self-match into groups. 

For those students who did participate in successful study groups, experiences were similar across demographic groups. High-comfort and high-activity groups were further associated with improved learning outcomes. While these findings might be explained by external factors, e.g., a student’s academic proactiveness and general social comfort may be associated with their better performance on exams, the positive associations are promising. The large scale of the experiment allowed us to have statistically significant conclusions in many (but not all) cases. 

Student scheduling and non-responsive students are two of the biggest obstacles to successful study groups. The majority of reassignment requests came from students whose initial assigned group members were non-responsive. We are improving our system to automatically send reminder emails to improve this issue. In some cases, there was a lack of leadership, where no one initiated meetings, which lead to the group not working out. We are considering explicitly asking students to self-identify as leaders in the initial preferences survey to address this. Many students also reported that they wished they had reached out to other students more, so active encouragement of this through guidelines and lecture might also be valuable. This all points to the need to have more active support during the semester for keeping the study groups active. While our current work does not focus on developing team dynamics, we hope to bring in best practices to encourage successful collaborations such as those in~\cite{oakley2004turning}.

The challenges around scheduling were surprising to us, since these were explicitly prioritized by the matching algorithm. We learned anecdotally that changing schedules and preferences on part of the students might be an issue here. This suggests an intervention where we might want to try slotting in ``study group time'' into official course schedules so that students who want to be in a group can block off that time when they sign up for courses.

%However, we learned anecdotally from students that schedules tend to change during the first few weeks and that students often have strong preferences on study times, and so offering a reassignment around this time might be one solution. We are also working on improving our system to automatically send reminder emails to students to improve the student responsiveness issues. Many students also reported that they wished they had reached out to other students more, so active encouragement of this through guidelines and lecture might also be valuable. This all points to the need to have more active support during the semester for keeping the study groups active.


%Students changing their mind about wanting to participate in study groups was likely the biggest challenge faced in the study. The overwhelming majority of reassignment requests came from students who never managed to meet with their assigned group members either because they were unresponsive to requests to meet, or students' schedules changed and they could no longer meet in the times they said they could. In some cases there was a failure through a lack of leadership --- no one decided to do the organizational work to get everyone together. We are considering multiple solutions to this based on other work on team formation --- e.g. explicitly asking students to self-identify as leaders in the initial preferences survey. Since the intake surveys were introduced on the first homework, students were only assigned study groups in Week 2, and one homework cycle has already passed by this time. An earlier intake survey might allow students to start collaborating right from the first homework, which could further encourage students to participate. 





%\TODO{Discussion:  However, given many students feel comfortable in groups and are not requesting reassignments, it could also be inferred that groups afford them the socio-academic support to exercise their academic proactiveness.}

%\TODO{We interpret this positively --- that with high confidence, the process of forming groups without racial or gender singletons enables underrepresented groups to have study group experiences on par with other groups, which was a major goal for us. 
%We did, however, notice some differences in study group outcomes based on student year; there are likely many reasons for this.

%We were not able to control against forming study groups through other methods, so we focus our analysis on normative statements to be made about experiences in our pilot group. We additionally do not draw any gender or race comparison conclusions about students who preferred not to state their gender or racial identity.


%\TODO{Discussion. These results support the decision to offer at least one reassignment along the course of a course term, as otherwise there may be students, occasionally disproportionately of underrepresented demographics, left with lower-quality groups from the outset. We also note in Section~\ref{section:grades_assoc} that never requesting reassignments can be associated with higher performance on exams. There may be different reasons for this and we do not have any insight into possibly hidden variables, so it is hard to establish any causality. However, we believe it is important to have a quick turnaround for reassigning groups to dissatisfied students.}





% \subsection{Student anecdotes} \label{sec:anecdotes}
% While we were unable to conduct systematic student interviews to understand the student experience beyond the surveys, some students voluntarily let us know about the impact the groups had on them, through written feedback regarding study group experiences after the end of the semester. Some notable anecdotes are below: 
% \begin{itemize}[leftmargin=5mm]
%     \item \emph{Starting my freshman year of college virtually due to the pandemic made me feel really disconnected from the Berkeley community, but luckily being a part of a study group for EECS16A in my first semester really changed that. As a woman and underrepresented minority in STEM, my study group gave me the support system necessary to succeed in an extremely rigorous and minority-isolating major. This group was essential when it came to having people to complete assignments, learn concepts, and study for exams with, but it was also very helpful in me finding life-long friends. Through my study group I met my first and closest friends at Berkeley who would help me adjust to college in an online world and who later became my supportive and caring roommates in my sophomore year of college.}
%     \item \emph{As a new transfer student beginning remote learning at Berkeley, my 16A study group had a massive impact on how I carried about my studies. Not only did meeting up with other students remind me how important team-work is within the field of engineering, but it was also a constant reminder that it is OK to struggle on problems before arriving at solutions. Our group worked really well together because we had shared experiences. 5/6 of us are transfer students, so we understand each other's strengths and weaknesses when learning new material. Some of my few, closest friends at Berkeley are my EECS16A/16B study group peers.}
% \end{itemize}

% Independent of any grade or learning improvements, just making even a few students have better and happier college experiences through study groups is valuable. We hope that at scale this can have a massive impact, which may or may not be measurable through numerical data.




%Specializing to freshmen, our largest but also one of our target demographics, we find even larger gains on exam scores for those who did not request reassignments. These results are especially promising given that over 75\% of freshmen never requested regroup assignments. 

%Finally, we explored the impact of study groups on students in different grade ranges. The most impact was seen in the B-range students. Students with B-range MT1 scores (between 68 and 89 percent, based on the class grading scale) saw significantly higher Final exam scores associated with high group interaction groups, and with feeling comfortable asking questions in the group. Additionally, knowing that the general distribution of Final scores was much lower than MT1 scores, students at the B range demonstrated significantly lower decreases from MT1 to the Final associated with several factors: frequently interacting groups, multiple group members participating, and feeling comfortable asking questions in their groups (Fig.~\ref{fig:ttest_groups}). These results suggest that for students who entered the class performing at a mid-level, being part of active and comfortable study groups benefited their grade. This range of grades constitutes a significant portion of the student population. 

%We also considered Students who received A, and C to below C-level, grades on MT1, but found no significant associations between their scores and group quality indicators. \TODO{This may be because students scoring at an A-level are well-prepared to succeed independently, and students with C-level grades may have external factors affecting performance and their ability to engage effectively with groups. }

%However, our findings above differed significantly when considering transfer students --- this demographic group had generally lower exam performance in general. In addition, students desiring to take courses with their group again, having higher group interaction in group, and having higher group member activity, tended to be associated with having lower exam scores. It is difficult to reason about this phenomenon, due to the large variability of transfer student backgrounds and personal situations.

==> SIGCSE 2023 arXiv Submission/sections/conclusion.tex <==
\section{Conclusion \& Future Work} \label{sec:conc_future_work}

The results presented in this paper stem from the Fall 2020 offering of EECS 16A at UC Berkeley. Since then, our research group has executed the matching process in numerous courses totalling over 3,000 students throughout the Spring 2021, Summer 2021, Fall 2021, and Spring 2022 semesters, and have had positive results based on preliminary looks at the data. A detailed analysis is yet to be conducted. Despite Fall 2021 and later semesters being in-person, we have found that study group formation continues to be in demand and well-used by courses. Student feedback has iteratively refined our process, and are experimenting with machine learning and reinforcement learning techniques to improve groups. We hope to soon release an open-source web-based privacy preserving version of our improved algorithm soon. 

==> SIGCSE 2023 arXiv Submission/sections/introduction.tex <==
\section{Introduction}
% Outline

% What is the problem? --- black students can't find study groups. Hypothesis: this is about structures and structural racism, and by using a new structure, we can support them. Won't fix all the issues, but will fix some of them. 
% What is your solution? A new structure
% Why is the problem important? Importance of groups and networks for learning and careers. 
% research questions
% Results 
%  summary/contributions
 
In 2013, a news outlet~\cite{eastbayexpress} ran a story about the University of California, Berkeley, %about UC Berkeley~\cite{eastbayexpress}, 
with a quote from the then director of the African American Student Development office:
\begin{quoting}[leftmargin=2mm]
\textit{``A black student might be in a science course, ... and the professor says, `Okay, everybody has to have a study group.' Nobody picks them for a study group. They first have to show that they can get an A before they get selected.''}
\end{quoting}
%
%Unfortunately, 
This problem still persists. In 2020 the president of the Black engineering students association at UC Berkeley~\cite{carlos} wrote: %\ref{doubleblind}]
%Black Graduate Engineering and Science Students at UC Berkeley recently wrote in 2020~\cite{carlos}:
\begin{quoting}[leftmargin=2mm]
\textit{``... I've stood by black CS undergrads who were constantly ostracized in group projects, often the last ones to be picked. Their peers regularly perceive them to be less knowledgeable and capable in carrying coding projects. I have had to console crying teenagers scarred from the experience, questioning, ..., whether being black was worth it. Imagine that. Their only path to recognition in that environment was through a bogus burden of excellence. What ever happened to the opportunity of being average yet respected?''}
\end{quoting}

%These quotes illustrate both the bias and extra challenges faced by Black students in forming study groups. 
These quotes illustrate some of the challenges faced by underrepresented students on college campuses. The social isolation of underrepresented students is a ``systemic problem''~\cite{hafferty2011can}. Additionally, underrepresented students can face an undue burden of excellence~\cite{hodge2008theorizing}, a burden of representing their demographic group~\cite{thompson2002being}, or stereotype threat~\cite{steele2011whistling}. In group settings, students may experience bias and microaggressions~\cite{grindstaff2019no, ong2011inside},  \emph{solo-status}~\cite{thompson2002being, spangler1978token} (\emph{i.e.}, be the only member of their demographic group present in an otherwise homogeneous group) or \emph{tokenism}~\cite{spangler1978token}. %Thus, it can be a much bigger burden for a student from an underrepresented group to initiate a study group as compared to a student from a majority group. 
%Anecdotally, women and students from other minoritized groups in STEM have shared similar challenges with the authors. 

Peer groups~\cite{turetsky2020psychological,  mishra2020social} and social networks~\cite{calvo2004effects, thomas2000ties} can have a large effect on the success of individuals. While some students come to college with a pre-established network, many students from underrepresented groups may not know other students when they start college. This, combined with the other factors mentioned, can make it much harder for a student from an underrepresented group to initiate a study group as compared to a student from a majority group. Despite the value of these study groups, many students simply do not have them. 
%flynn2016stem, palmer2011qualitative,

%~\cite{miles2020invalidated,lehman2022nevertheless}

\begin{table*}[t]
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
\textbf{Challenge} & \textbf{Approach to address challenge} \\ 
\hline
Study group initiation burden & Lightweight process, integrated into course structure \\ \hline
Bias & Uniform process for all students   \\ \hline
Solo-status & Algorithmically prevented \\ \hline
Microaggressions & Structured guidelines, instructor-initiated groups encourage professionalism
\\ 
 & Reassignment process offers agency and recourse in case of negative experiences\\
 \hline
 Stereotype threat &  No peer-evaluation or connection to grades \\
 \hline
\end{tabular}
\end{center}
\caption{Summary table indicating our approach to various challenges faced by students}
\label{tab:one}
\vspace{-8mm}
\end{table*}


% Challenge
%initiating study group ---> process for everyone, integrated into homework
%solo-status ---> no such groups permitted
%microaggressions in study groups ---> behavioral guidelines, intrsuctor mediated process encourages professionalism
%difficulty in ice-breaking ---> technical ice-breaker questions
%lack of agency ---> preferences, reassignment



%, and can feel isolated in technical courses~\cite{miles2020invalidated,hafferty2011can}.

We hypothesize that by providing a standardized structure for study group formation, we can mitigate some of the exclusion faced by minoritized students. Our goal is to help students in building long-term (one semester or more) study groups that evolve into friendships and support systems. For this, we design a process that is (1) \emph{scalable}, in that it can be used for classes with thousands of students with minimal instructor intervention, (2) \emph{inclusive}, in that it attempts to remove hurdles faced by underrepresented students in forming study groups, and (3) \emph{flexible}, in that it is opt-in and provides students the agency to request reassignment as desired. 
%
%Our experience is that students can face structural barriers from implicit bias because the onus is on them to initiate a study group. By providing a standard method for creating a study group, we remove this barrier and make the study group experience more equitable. 
%
%

\vspace{-4mm}
\subsection{Previous work on group formation}
%This project builds on a long history of work that identifies the importance of for students. 
 %While the social atmosphere at college supports student intermingling, this is not necessarily focused on building connections that support coursework, and this can lead to isolation in technical courses~\cite{}. 
%In some computer science departments, less than 10\% of the students may come from underrepresented groups\footnotemark[1]. 
%It is important to recognize this inequity and tackle it head-on. 
The fields of computer-supported collaborative learning (CSCL) and computer science education have explored various avenues for using technology to support student collaboration~\cite{wise2017visions, uttamchandani2020finding}. However, critics of CSCL point out that the tangible impact of the field has been small~\cite{wise2017visions}, and some~\cite{uttamchandani2020finding} urge the field to \emph{center on equity} to promote research that can make a difference. 

Forming good student groups is a complex multi-objective combinatorial optimization problem, where one must balance student schedules, personalities, skills, learning outcomes, instructor preferences, fairness and more. As a result, there has been tremendous work on different strategies and algorithms for group formation. Some recent surveys give an overview of much of the work around student teams~\cite{cruz2014group, odo2019group,putro2018group,borges2017group,maqtary2019group}. 
%
% There are many parameters to be considered in group formation and multiple variables can have an impact on the succes of the group,  Much of the work is focused on methods for composing groups,
For examples, some group formation strategies are based on topic-mastery and skills~\cite{deibel2005team, clarke1994pieces, dzvonyar2018team, mujkanovic2016improving, catme, hertz_2022}, others on problem-solving or learning styles~\cite{adan2011forming}, schedules~\cite{wills1994peer, dzvonyar2018team, catme, hertz_2022}, personality and interpersonal skills~\cite{lambic2018novel,mujkanovic2016improving}, and demographics~\cite{catme,hertz_2022, lovold2020forming}. Additionally, people have considered both algorithmic and machine-learning approaches to team formation~\cite{dzvonyar2018algorithmically, mujkanovic2012unsupervised, lambic2018novel}. Team assignments have been considered in the contexts of both final projects for MOOCs~\cite{staubitz2019graded, ju2018scalable} and short-term activities~\cite{srba2014dynamic}. Some of these works have also provided tools that can be used by others~\cite{catme, hertz_2022}.

At this point, we would like to make a distinction between \emph{study-groups} (that are informal, fluid, open-ended, and student-driven, e.g. meeting with friends in your dorm to work), from \emph{project-groups} (that are officially tied to grades, mandatory, inflexible, operate for a specific time, and have a predetermined focus). The prior work, including all of the works mentioned above, has largely focused on instructor-mandated groups that are assessment-focused, and are more like project groups than study-groups. In addition to considering group composition, they often focus on building teamwork skills in students. For instance, the most widely-used tool (8000+ instructors) is likely the CATME Teammaker~\cite{catme}. This team-formation software offers a built-in framework for peer-evaluation~\cite{aseepeer33497}. While such peer-evaluation can be very helpful for developing teamwork skills~\cite{ju2018scalable,oakley2004turning}, and can even improve grades~\cite{oneill2020team}, it can be difficult to implement effectively~\cite{van2010effective}, and can have negative implications for student relationships~\cite{zou2018student}. In the context of research-peer-reviews, unprofessional reviews may disproportionately harm underrepresented groups~\cite{silbiger2019unprofessional}. 
The focus on developing teamwork skills, and constantly being evaluated, can trigger stereotype threat and detract from the social support that a more informal study group would provide~\cite{mosley2007stigma}. %Lovold et al.~\cite{lovold2020forming} find that students who self-formed teams (based on students they already knew in the class) performed slightly better than those in instructor-formed teams, and hypothesize that the student comfort in self-formed teams is valuable. 

\emph{This work:} Our opt-in system builds non-mandatory (a student may choose to form their own group, ask us to form a group, or have no group at all) study groups, as opposed to project groups, with careful considerations for the experience of underrepresented students. A novelty of our system is that it offers students the chance to be reassigned to a new group after trying out a group for some time. We avoid groups where students may experience solo-status~\cite{thompson2002being}, and also consider intersectional identities~\cite{ Solomon2018NotJB, Rankin2020}. We also try to avoid homogeneous groups, given the importance of diversity in teams~\cite{hong2004groups}, and the value of increased social networks~\cite{calvo2004effects}. % Takeda_2014}.%, watson2002influence}.
%Rankin2021RealTS,
To the best of our knowledge, such optional (but instructor-generated) study groups that are not related to student assessment have not been studied extensively in the literature.

 % \paragraph{Group composition}
% Our group-formation algorithm builds on previous studies that identify structures of successful groups. Individuals experience \emph{solo-status} when they are the only members of their social category (e.g., gender or race) present in an otherwise homogeneous group. Many studies have shown the harmful effects of solo-status or tokenism in a group setting~\cite{thompson2002being, spangler1978token}, and highlight the importance of community and allies~\cite{born2020gender, powell2008improving,thompsonsystemic,zwolak2017students, turetsky2020psychological, palmer2011qualitative}. We avoid groups where students may experience solo-status,  At the same time, we try to avoid demographically homogeneous groups as well, given the importance of diversity in teams~\cite{hong2004groups, Takeda_2014, watson2002influence}.
\vspace{-3mm}
\subsection{Our contributions}
We design a lightweight system for study group formation that is integrated into the course structure and thus standardized for all students. We hypothesize that this reduces the \emph{structural barriers} faced by underrepresented students in creating study groups, while also supporting \emph{all} students. By creating instructor-supported but student-controlled opportunities for discussing coursework, we create opportunities for repeated interaction and proximity~\cite{rohrer2021proximity}, which can lead to friendship~\cite{preciado2012does}, while setting social norms that encourage positive interactions~\cite{koppenhaver2003structuring, dixon2009establishing}. The voluntary participation and ability to request reassignments gives students agency that can be essential in learning~\cite{stenalt2021does}. Table~\ref{tab:one} summarizes our approaches.% to various student challenges.

%We note that 
Large classes can be particularly advantageous for forming study groups, because small demographic groups can be amplified. In a class of 1000 students, if 30\% are women and 1\% are Black (approximate percentages at UC Berkeley), that is 300 women and 10 Black students. This scale allows for a flexibility in group formation that is not possible in a 100 student class with the same proportions. %possible in a 100 student class. 

We test our approach in a 1000+ student introductory undergraduate class in Engineering and Computer Science that was conducted remotely due to the COVID-19 pandemic\footnote{IRB approval for Protocol ID `2020-08-13526' and Approval Date `September 25, 2020.'}. The large course size allows us to compute statistically significant results in many cases, which is not possible in some of the smaller studies discussed earlier. Given the demographics in our classroom (typical for our institution), in this analysis we consider students identifying as women or gender non-conforming, as well as students identifying as Black, African American, Hispanic, Native American, Alaskan Native, Hawaiian Native (see numbers in Fig.~\ref{fig:self_form_comp}) as underrepresented. To support adoption of our system, all of the processes, surveys and code used for this process are available open-source~\cite{our_repo}, unlike systems such as CATME~\cite{catme}. 
%We obtained student consent and IRB approval of our human research protocol titled \textit{Creating positive experiences for first-year underrepresented students through scalable automated inclusive study group formation.}, with Protocol ID '2020-08-13526' and Approval Date 'September 25, 2020.'

\emph{Questions.} To understand if our system created positive experiences for underrepresented students, we ask the following questions.
(1) Who participates in the structured group formation process? Who participates in the reassignment process? (2)
Does the structured group formation process lead to students from minoritized and majority groups having similar experiences in their group interactions? (3)
Does the structured group formation process impact student performance on exams?







% Underrepresented students face challenges that impact their day to day interactions on the college campus. They report feeling isolated~\cite{hafferty2011can,miles2020invalidated,lehman2022nevertheless}, can face stereotype threat~\cite{steele2011whistling},  can face an undue burden of excellence~\cite{hodge2008theorizing}. Students may frequently experience \emph{solo-status}~\cite{thompson2002being, spangler1978token}, i.e. be the only member of their demographic group present in an otherwise homogeneous group, or be considered as \emph{token}~\cite{spangler1978token}. Thus, it can be a much bigger burden for a student from an underrepresented group to initiate a study group compared to a student from a majority group. 


%However, this focus on peer-evaluation detracts from the social support that is critical for students. Along with CATME, the majority of team-formation tools are focused on building teams that are mandatory (e.g. for final projects) or short-term (e.g. for a lecture exercise) ~\cite{mujkanovic2016improving,dzvonyar2018algorithmically,lovold2020forming, dzvonyar2018team,odo2019group,maqtary2019group,p,putro2018group,,staubitz2019graded,ju2018scalable, hertz_2022, srba2014dynamic, mujkanovic2012unsupervised, mujkanovic2016improving}. 







%The field of computer supported collaborative learning (CSCL) has deeply engaged with using technology to support learning however, the ``tangible impact of CSCL on educational practice is very small so far''~\cite{wise2017visions}.~\cite{uttamchandani2020finding} argue that ``centering on equity [in CSCL] will promote research that can make a difference.''

% We use a partitioning based algorithm that can provide better guarantees than the optimization approach used by CATME and other tools, as discussed further in the algorithm section~\ref{sec:algorithm}. Finally, the agency afforded to student through the reassignment option offered by our system is novel. 

%focuses on student-teams for projects, and can incorporate demographic constraints, schedule constraints, course-matching constraints and more. Instructors have the option to indicate how important each of these constraints are to them. In addition, this framework offers a suite of tools that can evaluate the performance of teams through peer-evaluation, for example as in~\cite{aseepeer33497}. Unfortunately, the full version of their work is not available open source. CATME uses a non-convex optimization problem on the backend to identify the groups, with a hill-climbing approach to finding the optimum. This approach likely only leads to the discovery of a local optimum, and while constraint violations may lead to a decrease in a team-score, and thus make the team less-likely to be chosen, the optimization framework cannot guarantee this. Our approach avoids this by using a partitioning approach.

%Their framework does not account for the added value of having  diversity across race and gender in teams, which we are building explicit checks for. Another tool of note is Gruepr, which builds on CATME but provides an open-source implementation~\cite{hertz_2022}. However, their algorithm only works for partitioning up to 300. students at a time, while ours scales to 1000's of students. It uses a genetic algorithm to explore the optimization landscape --- with a large number of random seeds it has a chance to avoid local optima. However, one still cannot provide guarantees of constraint non-violation. Our partitioning based approach allows us to prioritize certain constraints over others as deemed important by the instructor, with is different from the optimization approach of CATME and Gruepr.

%by explicitly pairing students who share race/gender identities. Given the importance of intersectional identities, the system also considers these in the pairing. At the same time, we also a studies have shown that diversity in teams can also be valuable~\cite{hong2004groups, Takeda_2014, watson2002influence}. As a result, our algorithm avoids creating homogeneous groups.%, which can also create important broader social networks for students~\cite{calvo2004effects,calvo2004job}.






% We consider our proposal in the context of the framework for campus racial climate developed by Hurtado, Milem and colleagues~\cite{hurtado1998enhancing}. While the majority of campus initiatives to support diversity often focus on compositional diversity (they numerical/proportional representation of groups),~\cite{hurtado1998enhancing, milem2005making} point out that the historical legacy of inclusion/exclusion, the psychological and behavioral climate, and the organizational/structural aspects really matter. Our intervention attempts to link the 
% behavioral dimension with the organizational/structural dimension through course instructor facilitated structured study groups. 

%\paragraph{Questions}
%This paper provides an algorithm for study-group formation and investigates the impact of the structured group formation process on students. 
%We hypothesize that by having the group-formation process be standard and equally accessible to all students in the classroom, we will remove some of the structural barriers faced by students from underrepresented groups and provide positive experiences. We ask the following questions: 


%\begin{itemize}
   


%We tested%Our protocol, \textit{Creating positive experiences for first-year underrepresented students through scalable automated inclusive study group formation}, with Protocol ID '2020-08-13526' was approved by the UCB CPHS office on 'September 25, 2020.'} 
%our system in a 1000+ student freshman class that was offered entirely remotely during the COVID-19 pandemic. 

%\paragraph{Main contributions}
%This paper discusses the development of a scalable survey and software system to generate long-term study groups. A key feature of our system allows students to `try out' a study group for a few weeks and then request a reassignment to a new group if their first group is not working out for them. They may do this multiple times throughout the semester. This gives the system and course instructors the opportunity to improve group matches over time and improve the student experience, and sets up a system by which our system can \emph{learn} better groups over time. 

%Our matching system can considers multiple concrete factors (e.g. student schedules, demographics) as well as factors such as student motivation in generating the groups. We build on previous works such as~\cite{catme, hertz_2022}. These works identified that solo/singleton status (students who are the only representative of a given demographic in their study group) in a group may harm students. However, the optimization-based frameworks of~\cite{catme, hertz_2022} are likely to avoid solo status, but cannot guarantee it. Our partitioning based system (see Sec.~\ref{subsec:multi-partitioning}) can provide guarantees for this. In addition, our matching system and code can scale to thousands of students, unlike ~\cite{hertz_2022}. Our code will also be available open-source at~\cite{our_repo}. Our focus is on a system for voluntary long-term student interactions, without any connections to grades, and we build other infrastructure (e.g. guidelines for study-group operation, discussion-based homework problems, and more in Sec.~\ref{sec:timeline}) to support this. This contrasts with the shorter-term project focus that other systems may have.

%In evaluating our system, we offer a case study of the impact of study groups during the first exclusively remote semester at UC Berkeley. We find that most (over 50\%) of the students in groups we assigned had positive experiences across four of five quality indicators (see Sec.~\ref{sec:overview_impact}). Notably, more than 74\% were comfortable asking questions and sharing ideas in their groups (see Sec.~\ref{sec:overview_impact}). We find that our system was particularly useful to students from underrepresented demographic groups --- these students were more likely to request a study group via our system than form their own study groups (see Sec.~\ref{sec:self_formed_comp}). Furthermore, for those students who were matched into groups by our system, we find that students of underrepresented race and gender demographics had similarly positive study group experiences to majority groups (see Sec.~\ref{sec:dem_comparisons}). In analyzing group associations with academic performance, feeling comfortable sharing ideas and asking questions in study groups was significantly associated with increased midterm scores (see Sec.~\ref{section:grades_assoc}). 






%%%%%%%%%%%%% COMMENTED OUT STUFF BELOW HAS ALREADY BEEN INCORPORATED



% The details of the social support matter very much, and the specific composition of a study groups can also have a great impact on their dynamics. Individuals experience "solo status" when they are the only members of their social category (e.g., gender or race) present in an otherwise homogeneous group. Field studies and surveys indicate that members of socially disadvantaged groups, such as women and racial minorities, have more negative experiences as solos than members of majority groups, such as white and male-identifying students~\cite{niemann1998relationship}. Solo status can lead to lower public performance, which hurts retention of women and racial minority students \cite{thompson2002being}. Tokenism, or perfunctory/symbolic efforts to be inclusive to members of underrepresented groups~\cite{kanter1987men}, can lead to poor performance of students from the underrepresented groups~\cite{spangler1978token}.~\cite{thompsonsystemic} highlights that retaining women in undergraduate computing can be facilitated through collaborative learning in classrooms by creating a sense of community. In fact, a study about improving the persistence of first-year undergraduate women in computer science showed that women appreciated all-women support groups because they provided opportunities to discuss academic and social issues concerning the major~\cite{powell2008improving}. In another study, women who were randomly assigned to male majority teams were less willing to become team leaders than women assigned to women majority teams \cite{born2020gender}. It is further important to consider intersectional identities in this~\cite{Rankin2021RealTS, Solomon2018NotJB, Rankin2020}. This literature leads us to strongly believe that we should ensure that no students experience solo or singleton status in study groups.

%%At the same time, homogeneity in groups is not necessarily ideal. We know that broader networks that go beyond self-identified student affinity groups are better for student retention and success~\cite{thomas2000ties}. Furthermore, the work of Hong and Page~\cite{hong2004groups} tells us that diverse groups of problem solvers can outperform high-ability groups. Many other works also emphasize the importance of diversity in groups~\cite{Takeda_2014, watson2002influence}. Thus it is important that students not get siloed into interacting only with students from familiar racial, ethnic and gender identities and learn to effectively interact across these groups. 

%Group work is an important component of engineering, where many projects (both at the university level and in real-life) are team-based. Students often form informal study groups to work on homework problems, study for exams, and do course projects. %Astin's influential paper calls out the student peer-group as the most important environmental influence on student development~\cite{astin1997matters}. 

%However, the move to online learning due to the COVID-19 pandemic made it significantly more challenging for students to meet each other and work together~\cite{wut2021person, whitley2021, engzelle2022376118}. And even under pre-pandemic circumstances, study groups have not been equally available to all students. Students from underrepresented communities struggle to make essential social connections and study-groups and may feel excluded~\cite{spangler1978token, niemann1998relationship, buzzetto2010unlocking, amelink2018exploring, Raabe2019, chen2019women, born2020gender, thompson2002being}. This is particularly true at UC Berkeley where our introductory classes often have 1000's of students, and very small numbers of students from certain groups (e.g. less than 10 Black students in a class of 1000).


%To address these challenges, we designed a flexible, inclusive, and scalable custom software solution to automatically group students based on their preferences while enforcing inclusive group formation. Our focus here is on developing an end-to-end system that can be used to develop long-term study groups (for one course or more). We distinguish study-groups (which are informal, fluid, open-ended, and student-driven) from project-groups (which are officially tied to grades, fixed, and have a predetermined focus). Our goal is to have long-term (one semester or more) study groups that evolve into friendships and support systems, not just groups to work on a particular assignment or project. With this perspective, group reassignment based on feedback from students is a key feature of our system, and this distinguishes our work from other approaches~\cite{catme, hertz_2022}.


%We first trialed our system in an introductory Electrical Engineering and Computer Science (EECS) course at UC Berkeley, consisting of over 1,000 students, and it has subsequently been used in multiple other lower-division and upper-division courses in the EECS department. The online semester provided a unique opportunity to study the impact of intentional and structured study groups for students, since the natural in-person social process by which students form study groups was disrupted.


%\textbf{Social support in the classroom:}
%Social support matters everywhere, and especially in the classroom. It has been shown that socially-connected employees are less likely to quit or change their jobs~\cite{mossholder2005relational, moynihan2008ties}. Social-networks can encourage individuals to persist in challenging environments where they might otherwise drop out~\cite{moynihan2008ties}. 
%Social integration, institutional commitment, and intention matter in students' retention, and students with broader, well-connected networks are more likely to persist in college~\cite{thomas2000ties}. Similarly, students' friends' retention was found to have a large impact on their own retention~\cite{eckles2012social}, and their integration into the social network matters as well~\cite{zwolak2017students}. Simple psychological interventions that improved social connectivity in the classroom have also increased retention~\cite{turetsky2020psychological}. Anxiety in the classroom can be mitigated to some extent by feelings of interpersonal familiarity and acceptance by peers \cite{varma2006making}.

%Most students entering university in Fall 2020 did not have access to the usual meetups, orientations, or events that allow them to develop these social support networks. This widens the divide between those who come to Berkeley from feeder schools (where multiple students from the same school/community college are in university together), versus those who are the only representative from their school/area. Based on student interviews, we know that students from underrepresented groups are less likely to have extensive peer networks when they come to Berkeley. This made it imperative that we institutionally help students find social support and peer groups. For many first-year students, the study groups were one of the few ways they connected with others. This also made it important to indicate to students that these groups are not limited to working on specific projects, but are really opportunities for them to develop relationships with their peers.












==> SIGCSE 2023 arXiv Submission/sections/methods.tex <==
\section{Methods}

\subsection{High-level system description}
Our system design was informed by informal informational interviews with cultural and identity-based STEM student organizations%\footnote{Black Engineers and Science Students Organization (BESSA), the Society of Women Engineers (SWE), Computer Science Scholars, the Hispanic Students Society (HES) and the Transfer Students Pre-Engineering Program (TPREP).} 
and the Director of Student Diversity in our department. Given their informal nature, we do not report on the interviews here. Students mentioned that one of the biggest challenges is trying to find people to work with when many other students already have connections with each other. It was also mentioned that it can be difficult for women to find women-majority groups to work in, that scheduling times for study-groups is hard, and microaggressions in study groups can lead to people wanting to work alone. The Director of Student Diversity emphasized the longer-term impacts of study-groups such as influencing post-graduation decisions as well as increasing enjoyment in education.

%Since our main aim with this system was to reduce structural barriers for students in forming study groups, 
We focused on a process that was simple and low-overhead. There were no grade incentives associated with joining groups. The process was opt-in, and the students had the choice of forming their own groups (we call these \emph{self-matched} groups), asking us to form a group for them (we call these \emph{software-matched} groups), or having no group at all.

\paragraph{Timeline} Students opted-in to be matched to a group through a survey on their first homework assignment in Week 1. Reassignment rounds were conducted in Weeks 5 and 9, where students were invited to request new groups by updating their survey preferences if they were not happy with the first group they were matched to. This was also an opportunity for students to provide feedback on the matching process/ group experience thus far. A final evaluation survey to collect student feedback on their experience was released in Week 13, through the final homework.

\paragraph{Group-creation survey} \label{sec:survey-design}
Groups were created based on students' scheduling preferences and other information, collected in Week 1. In particular, the student survey collected information about (1) current timezone (our students were distributed around the globe due to COVID-19), (2) preferred meeting days, (3) preferred meeting times on those days, (4) year (\emph{e.g.,} freshman, sophomore etc.), (5) other courses taken in the current semester (to maximize overlap), (6) whether student previously took a linear algebra or a coding class, (7) preferred discussion section time (so students could attend the same discussion section), (8) how important the course is to the student, and  (9) gender and race identity. Questions (7), (8) and (9) were optional. Students were encouraged to select-all-that-apply for scheduling questions to maximize matching potential, so someone that is free on both Monday and Tuesday would select both options. The exact surveys for group-creation and evaluation, and the group guidelines discussed below are available at~\cite{our_repo}. 
%[specific class related to the course\footnote{Removed for double-blind review, but will be included in the final version.\label{db2}}]



% A Black male student mentioned that the biggest challenge is being in a classroom where many students already have connections with each other and trying to figure out people to work with. This can be an overwhelming experience, especially in a large class. 

% Two female Hispanic students mentioned that finding study groups is not difficult but having a functional study group can be challenging. One of them highlighted that “it is easy to meet some people in office hours who are seeking help and ask to work with them. However, scheduling meeting times might be hard after that.” 

% A Black female student mentioned that the conduct of team members makes it hard to work with some students. “Too many micro-aggressions and hence the need to work alone after that.” This student narrated her experience that showed that study groups formed randomly in a class section could end up hurting the students if they lack proper guidelines on how to collaborate. 

% A female Indian student mentioned that being in majority male study groups makes it hard for her to speak up because the men constantly try to take credit for everything she says. She mentioned that it had been hard for her to find majority female study groups given the low numbers of women in the Computer Science department.

% The Director of Student Diversity emphasized what most of the students said. Through speaking with the Office of Student Diversity in EECS, we learned that many students need their peers for support in not only classes but also to enjoy learning the material. Study groups can also influence post-graduation decisions, such as going to graduate school. We also learned that students who do not feel isolated enjoy their time at Berkeley a lot more than students who feel alone.


%\TODO{This included information about their current timezone, preferred meeting days and times, their coursework background, their year, as well as optionally, their race and gender identity. We also asked students how important the course was to them, what other courses they are currently taking, and their preferred discussion section attendance times (to allow students to attend discussion section together if possible). No skills or GPA information.}


\paragraph{Supporting in-group interactions} Following work such as~\cite{oakley2004turning}, we released a set of guidelines for collaboration~\cite{our_repo}. This included rotating role-assignments (Facilitator, Timekeeper, Librarian, Scribe) and suggestions for the meeting structure. %The full guidelines are available here~\cite{our_repo}. %[reference removed for double-blind review, will be included in the final version].%~\cite{16a_fa20_group_guidelines}. 
Additionally, we designed new open-ended homework questions to encourage discussion and sharing of ideas as coursework-related ``ice-breakers.''% for the groups.

\subsection{Evaluation survey} \label{sec:evalsurvey}
We evaluated the student experience using a survey~\cite{our_repo} in Week 13. %Specific questions are available [here]\footnotemark[3]. %~\cite{16a_fa20_evals}. 
Five questions related to the quality of the study group experience for each student: (1) the comfort of the student in asking questions in their group, (2) the comfort of the student in sharing ideas with their group, (3) the interaction frequency (how many times a week did they interact), (4) the number of students in the study group that regularly participated, and (5) whether the student wants to take future courses with their group. We also collected information about the number of reassignments requested by students and the obstacles they experienced in the success of their study groups. %We were also interested in understanding associations with how many times a student requested reassignment to a new group. 

\subsection{Group formation algorithm} \label{sec:algorithm}
As discussed earlier, group formation is a multi-objective optimization problem with fairness and resource constraints. There are no clear optimal strategies for this problem, and multiple approaches such as greedily maximizing heuristics ~\cite{catme,odo2019group},  genetic algorithms~\cite{hertz_2022}, clustering approaches~\cite{odo2019group}, similarity maximization~\cite{odo2019group}, and more have been tried. Here, we choose to take a partitioning-based approach with an explicit priority-ordering of the constraints, instead of an indirect prioritization through an optimization heuristic. %Our algorithm is not optimal, 
%We take a partitioning-based approach instead of the optimization-based approach taken by works such as CATME~\cite{catme} and Gruepr~\cite{hertz_2022}. This approach allows us to provide stricter guarantees on the groups, as opposed to the hill-climbing approaches in~\cite{catme, hertz_2022} that converge towards locally-optimum solutions and make looser trade-offs.

At a high-level, our algorithm repeatedly partitions the class based on scheduling and course-matching constraints, and then ensures that group-composition demographic constraints are met in the formed groups. %To maximize matching flexibility while keeping the groups a reasonable size,
We formed groups of four to six students~\cite{oakley2004turning}, with some exceptions to maximize matching flexibility and avoid solo-status. %The majority of the groups were five to six students each. % Our goal was to form study groups sized between four to eight students --- we allowed this flexibility in size for greater matching freedom. %The general algorithm and process is outlined in Fig.~\ref{fig:flowchart}. 
The algorithm is divided into three phases: (1) Multi-partitioning, (2) Tentative group assignment, and (3) Finalizing group composition to avoid solo-status. %Each phase of the algorithm is explained as follows.


\label{subsec:multi-partitioning}
\textbf{Multi-partitioning:} 
\input{figs_code/partition_tree_example}
Multi-partitioning repeatedly partitions the class until all matching criteria are exhausted. For Fall 2020, we used the following priority-ordered partitioning sequence: (1) timezone, (2) meeting day, (3) meeting time, (4) class year, (5) courses this semester, (6) previous courses, (7) discussion time, and (8) course importance. If some of the partitions are too small (less than four students), they are merged into the nearest neighboring partitions (distance computed as edge hops on the partition tree). 

Student schedules are the most important constraint. To maximize matching flexibility, we allow a student to be provisionally placed into \emph{all} the partitions that their schedule allows. For example, someone who is free on Monday morning, Monday afternoon and Tuesday afternoon would be provisionally placed in all three partitions. Fig.~\ref{fig:multi-partition_tree} shows an example of the tree formed by this process, using student timezone as the first partitioning criterion and then meeting day as the second criterion. Duplicates are handled after tentative group assignment: once a student is assigned to a group, they are removed from all other partitions.


%This duplication is handled later through considering the partitions in a specific order. 

%While this partitioning approach would ensure that no constraints are ever violated, strict partitioning can be too restrictive when it comes to select-all-that-apply questions, which is why we use multi-partitioning. For example, consider a scheduling constraint, where students are asked to choose days of the week when they would prefer to meet. In implementing multi-partitions for this criteria, students are included in \textit{all} of the subdivisions where they could feasibly meet. Thus, a student who indicated either Monday or Wednesday would work for them would initially be placed in both subdivisions simultaneously. 


\textbf{Tentative group assignment:}
%We consider the partitions in a specific order to ease the group creation. 
We iterate over the partitions to assign groups. We first assign groups in the smallest partitions that are ``just right,'' \textit{i.e.,} those with four to six students in them. Once a group is formed, the corresponding students are removed from all other partitions. If the group assignment causes a partition to dip below the smallest viable group size, the partition is merged into the nearest neighboring partition. Partitions are considered in increasing order of size after that. In partitions with multiple groupings possible, groups are formed randomly. % within the partition. 

%To avoid assigning a student to multiple groups, we create groups in a very specific order. We first identify all partitions that are already of the right size to form study groups, i.e. have four and eight students in them. Partitions with less than four students are merged to form larger partitions. 
%iterate over all subdivisions in a heuristically-defined order and remove students who are placed in multiple partitions. 
%Our heuristic prioritizes partitions that are of the correct size to form a group themselves.

%Then, we consider partitions of increasing sizes, until all partitions are assigned. 
%To do this we define a range (a `window') of partition sizes that are finalized first and keep expanding the range until all partitions are assigned. In doing so, we strike a balance between the common most-constrained-value and least-constrained-value heuristics, because otherwise, very small or very large groups tend to be created. In the earlier example, if Tuesday afternoon is iterated over first per the heuristic, then the student above is maintained in that partition but removed from Monday morning and Monday afternoon. 
%We then iterate over subdivisions and prune other copies of the students in order to achieve well-balanced partitions. For example, if the Monday partition is substantially larger than the Wednesday partition, then students who indicated both availability would preferentially be maintained in the smaller Wednesday partition.



%After multi-partitioning on the hard-constraints is complete, students are further partitioned based on the remaining constraints (i.e., the questions (6) discussion time, and (7) course importance), which we consider as soft-constraints and permit students to not match on these. 
%Within each partition, students are clustered into affinity groups based on their information. We sequentially form "soft" clusters of students based on criteria not used for partitioning such as demographics, other enrolled courses, motivation in the course and so on. 

%Students are partitioned based on these questions as long as the number of students in a partition does not go below four. If the partition gets too small, the process stops and a study group is created. 


%Students are similarly partitioned as described earlier so as to maximize overlap. Once all the partitioning  These clusters are then split into study groups that obey the sizing constraints, although groups may be formed across cluster boundaries if necessary.

\textbf{Finalizing group-composition to avoid solo-status:} %Since the earlier clustering is done in a soft manner, it does not provide any hard guarantees.
The last step in the algorithm considers the racial and gender identities of the students in the groups. In particular, it is at this stage that we ensure that no students have solo-status (\textit{i.e.,} are the only member of their race or gender) in their groups. To achieve this, the algorithm iterates over all groups to identify any students with solo-status. Students with solo-status are removed from their tentative assignments and %\footnote{We consider solo-status students from both minoritized and majority demographics.}, 
partnered into pairs or triples of students who share the same gender and race identities, while considering intersectional identities. If suitable partners cannot be found within the partition, we allow partnering outside the partition. Once the pairs/triples in each partition are generated, they are randomly merged with another pair/triple to create a study group. We first search within the partition for a pair/triple to merge with, but if none exist, we extend our search to other neighboring partitions. 
Since the course composition may be such that it might not be possible to avoid solo-status for \emph{all} students (\textit{e.g.,} if there is only one student from a particular racial group), this process is stopped after the number of students with solo-status is below a configurable threshold.
%
Finally, we manually checked to ensure that there were no racially-homogeneous groups~\cite{hong2004groups} (some gender homogeneity is unavoidable), which turned out to be the case. However, this is not always guaranteed. %Subsequently this check has been incorporated into future versions of the algorithm. 
%However, given the demographics of the student body --- where there are a large number of men and Asian students --- it was not possible to guarantee non-homogeneity for all groups, and some groups from our majority demographics were homogeneous.
Our code is available at~\cite{our_repo}. 
% The algorithm is roughly sketched as Algorithm~\ref{alg:cap}. We omit some of the corner cases in the summarized presentation for clarity. 



% \begin{algorithm}[t]
% \caption{High-Level Grouping Algorithm Summary}\label{alg:cap}
% \begin{algorithmic}
% \State $S$ \Comment{$S$: students}
% \State $G \gets \texttt{\{\}}$ \Comment{Initialize empty list of groups}
% %\For {constraint $c$ in $C$}
% \State $P \gets$ \textbf{Multi-partition}$(S)$
% %\For {student $s$ in $S$}
% %     \State $P \gets$ \textbf{Multi-partition}$(s, P)$
%      %\State $s$.assigned $\gets 0$ \Comment{All students initially unassigned}
% %\EndFor
% %\If {$c$ is SchedulingConstraint}
% %    \State $P \gets$ \textbf{Prune}$(P)$ %\Comment{Remove duplicate student instances}
% %\EndIf
% %\EndFor
% %
% %\State \textbf{Order}(P) \Comment{Order partitions using heuristic described in \S\ref{sec:algorithm}}% as described}
% %
% \For{partition $p$ in P} %\Comment{hard constraints \textit{e.g.,} timezone=PST}
%     \State $L \gets$ [all unassigned students in partition $p$]% and $s$.assigned $= 0$]
%     \If {$|L| \leq \texttt{upper}$} \Comment{upper = 6}
% \State $G.\operatorname{append}(L)$ \Comment{Assign $L$ as a group}
%     %\For {student $s$ in L} $s$.assigned = 1 %\EndFor
%     % \ElsIf{$|L| < \texttt{lower}$}
%     %     \textbf{Merge}(p, P) \Comment{Merges $p$ with other small partition}
%     \Else \State $G.\operatorname{concat}$(\textbf{RandomizeGroups}$(L)$) \Comment{Create randomized groups within partition and add to $G$}
%     %\For {student $s$ in L} $s$.assigned = 1
%     %\EndFor
%     \EndIf
% \EndFor
% % \State $\texttt{S} \gets \texttt{[]}$ \Comment{Track final subgroup assignments.}
% % \For{\texttt{tentative assignment $L$} in $G$} \Comment{In a heuristic-defined order}
% %     \State Remove instances of students in $L$ from assignments in $S$.
% %     \State Form subgroup \texttt{currSG} with remaining students
% %     \State $\operatorname{append}\left(\texttt{S}, \texttt{currSG}\right)$
% % \EndFor
% % \State $\texttt{allSC} \gets \texttt{[]}$ \Comment{Track all soft-clusters, across leaves}
% % \For{\texttt{subgroup $L$} in $S$}
% %     \State \texttt{Perform "soft" divisons in $L$:} Use non-rigid criteria to form soft-clusters \texttt{currSC} within each leaf node.
% %     \State $\operatorname{append}\left(\texttt{allSC}, \texttt{currSC}\right)$
% % \EndFor
% \While{solo-status count $<$ threshold} %\Comment{Stops if the violation count no longer decreases each iteration}
%     \State $Q \gets$ [all partitions with any solo-status members]
    
% \For {partition $Q$}
%     \State $R, H \gets$ [students, groups with solo-status in $Q$]
%     \For {group $h$ in H}
%     \State $U \gets$ [students with solo-status in $H$] 
%     \State $H.\operatorname{remove}(U)$
%     \EndFor
%     \State $T \gets$ \textbf{Partner}$(R)$ \Comment{Create pairs/triples among students}% This may violate soft-constraints}
%     \State $G.\operatorname{concat}$(\textbf{RandomizeGroups}(T)) \Comment{Randomly merge pairs/triples to form groups}
% \EndFor    
%     %\State \texttt{Select a solo-status individual or individual from homogeneous group}
%     %\State{Regroup to minimize violation count}
% \EndWhile

% \end{algorithmic}
% \end{algorithm}







% \begin{algorithm}
% \caption{High-Level Grouping Algorithm Summary}\label{alg:cap}
% \begin{algorithmic}
% \State $G \gets \texttt{\{\}}$ \Comment{Hold tentative subgroup assignments.}
% \For{\texttt{path $P$ in layers tree}} \Comment{\textit{e.g.,} timezone=PST, student year=sophomore}
%     \State $S \gets \texttt{[all students who fall under path $P$]}$
%     \State $G[P] \gets S$ \Comment{Note that this loop is implemented recursively to obey a partition limit}
% \EndFor
% \State $\texttt{S} \gets \texttt{[]}$ \Comment{Track final subgroup assignments.}
% \For{\texttt{tentative assignment $L$} in $G$} \Comment{In a heuristic-defined order}
%     \State Remove instances of students in $L$ from assignments in $S$.
%     \State Form subgroup \texttt{currSG} with remaining students
%     \State $\operatorname{append}\left(\texttt{S}, \texttt{currSG}\right)$
% \EndFor
% \State $\texttt{allSC} \gets \texttt{[]}$ \Comment{Track all soft-clusters, across leaves}
% \For{\texttt{subgroup $L$} in $S$}
%     \State \texttt{Perform "soft" divisons in $L$:} Use non-rigid criteria to form soft-clusters \texttt{currSC} within each leaf node.
%     \State $\operatorname{append}\left(\texttt{allSC}, \texttt{currSC}\right)$
% \EndFor
% \While{\texttt{constraint violation count $<$ threshold}} \Comment{Stops if the violation count no longer decreases each iteration}
%     \State \texttt{Select a solo-status individual or individual from homogeneous group}
%     \State{Regroup to minimize violation count}
% \EndWhile

% % \State $MP \gets \texttt{[MP groups]}$
% % \While{$N \neq 0$}
% % \If{$N$ is even}
% %     \State $X \gets X \times X$
% %     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% % \ElsIf{$N$ is odd}
% %     \State $y \gets y \times X$
% %     \State $N \gets N - 1$
% % \EndIf
% % \EndWhile
% \end{algorithmic}
% \end{algorithm}






==> figs_code/boxplots_race.tex <==
\begin{figure}[h]
    \centering
    \includegraphics{figs/race_dem_errorbars.png}
    \caption{Comparisons, between students identifying with differing races, in percentages ($y$-axis) answering positively to key study group quality questions. Students of mixed race were counted multiple times, in each of the racial categories they indicated they identified with. }
    \label{fig:race_boxplots}
\end{figure}

==> figs_code/boxplots_year.tex <==
\begin{figure}[h]
    \centering
    \includegraphics{figs/year_dem_errorbars.png}
    \caption{Comparisons, between students of differing years in undergraduate study, in percentages ($y$-axis) answering positively to key study group quality questions. }
    \label{fig:year_boxplots}
\end{figure}

==> figs_code/demographic_boxplots.tex <==
\begin{figure*}
    \centering
    \includegraphics{figs/gender_dem.png}
    \includegraphics{figs/race_dem.png}
    \includegraphics{figs/year_dem.png}
    \caption{Comparisons between students of differing demographics, in percentages ($y$-axis) answering positively to key study group quality questions, and counts (displayed on bars) answering positively to key study group quality questions. For student race, students of mixed race were counted in each of the racial categories they indicated they identified with. }
    \label{fig:dem_boxplots}
\end{figure*}

==> figs_code/img_matching_flowchart.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/flowchart.pdf}
    \caption{
        \label{fig:flowchart}
        Group matching process flowchart along with a detailed software diagram (in gray). First, students are routed based on whether they want a study group and whether they already have a self-matched group in mind. For the remainder of students, our software uses the student preferences to match them into groups. The algorithm first partitions students based on the most important criteria, forms groups within subdivisions to maximize matches on secondary criteria, and finally then performs checks on the demographic and preference-based breakdown within each group. After ensuring that no singletons are present and performing additional verification, the resulting groups are finalized and displayed.
    }
\end{figure}

==> figs_code/img_matching_timeline.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/timeline.pdf}
    \caption{
        \label{fig:timeline} The timeline of the group assignment process, from initial surveys to the final evaluation, in the context of the homeworks and exams in the class.}
\end{figure*}

==> figs_code/positive_response_correlation_matrix.tex <==
\begin{figure}
    \centering
    \includegraphics{figs/indicator_corrs.png}
    \caption{Pearson correlation matrix of positive responses to study group quality indicators.}
    \label{fig:indicator_corrs}
\end{figure}

==> figs_code/table_grade_assocation_confidence_intervals.tex <==
\begin{figure*}

\centering
\begin{tabular}{llllll}
  \textbf{Student group} &
  {\begin{tabular}[c]{@{}l@{}}\textbf{Indicated positive response to question} \\ \textbf{/ did not indicate positive response}\end{tabular}}  &
  {\begin{tabular}[c]{@{}l@{}} \textbf{MT1 Score} \\ \textbf{(Max 50)} \end{tabular}} &
  {\begin{tabular}[c]{@{}l@{}} \textbf{MT2 Score} \\ \textbf{(Max 50)} \end{tabular}} &
  {\begin{tabular}[c]{@{}l@{}} \textbf{Final Score} \\ \textbf{(Max 100)} \end{tabular}} &
  \textbf{Misc. diff} \\ \mytoprule
\multicolumn{1}{|l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\textbf{All software-matched} \\ \textbf{students}\end{tabular}}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Did not request reassignment\\ / did request reassignment 1-3 times\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.27 / 37.71 \\ ( p=0.003)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.72 / 36.42 \\ (p=0.025)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.01 / 67.35 \\ (p=0.046)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable asking questions \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.68 / 36.22 \\ (p=0.022)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.22 / 66.08 \\ (p=0.011)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable sharing ideas \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.04 / 37.60 \\ (p=0.011)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.81 / 35.27 \\ (p=0.002)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}71.96 / 65.86 \\ (p=0.046)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \mytoprule
\multicolumn{1}{|l|}{\textbf{Freshmen}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Did not request reassignment\\ / did request reassignment 1-3 times\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}41.40 / 37.60 \\ (p=0.0006)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.44 / 37.17 \\ (p=0.007)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}74.56 / 68.55 \\ (p=0.046)\end{tabular}} &
  \multicolumn{1}{l|}{-} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable sharing ideas \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}40.96 / 37.41 \\ (p=0.009)\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} \\ \mytoprule
\multicolumn{1}{|l|}{\textbf{Transfer}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Would take future courses with group \\ / would not\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}32.00 / 39.57 \\ (p=0.001)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}61.02 / 73.71 \\ (p=0.012)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}MT1-MT2: \\ -0.075 / 0.012 \\ (p=0.018)\end{tabular}} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Any group interaction \\ / no interactions with group\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}34.96 / 39.43 \\ (p=0.013)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}32.45 / 38.98 \\ (p=0.005\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}61.65 / 72.81 \\ (p=0.030)\end{tabular}} &
  \multicolumn{1}{l|}{} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Some to most members participated \\ / no members participated\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}35.64 / 39.31 \\ (p=0.024)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}} 33.08 / 39.16 \\ (p=0.009)\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} \\ \mytoprule
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Students receiving a} \\ \textbf{B-, B, B+ on MT1}\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Any group interaction \\ / no interactions with group\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.71 / 65.78 \\ (p=0.008)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}MT1-Final: \\ -0.075 / -0.14 \\ (p=0.003)\end{tabular}} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Some to most members participated \\ / no members participated\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}-0.084 / -0.130 \\ (p=0.047)\end{tabular}} \\ \cline{2-6} 
\multicolumn{1}{|l|}{} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Felt comfortable asking questions \\ / did not\end{tabular}} &
  \multicolumn{1}{l|}{-} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}38.99 / 36.53 \\ (p=0.044)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}72.18 / 63.91 \\ (p=0.004)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}-0.082 / -0.154 \\ (p=0.004)\end{tabular}} \\ \mytoprule
\end{tabular}
\caption{
        \label{fig:ttest_groups}
        Student's t-tests on difference in sample means, between exam grades within demographic groups, split on positive/negative responses to group experience indicators in the group survey. Only cells with significant differences in sample means are highlighted, with p-values provided. The Miscellaneous Differences column contains percentage-score changes for a student group, either from Midterm 1 to the Final, or from Midterm 2 to the Final, as indicated. Final scores were overall lower than midterm scores, so lower decreases in percent scores are interpreted as positive results.  
    }
\end{figure*}

==> figs_code/table_positive_response_students.tex <==
\newcommand{\mytoprule}{\specialrule{0.15em}{0em}{0em}}
\begin{figure}
    \centering
    \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Group Quality Indicator} & \textbf{Software-Assigned} & \textbf{Self-Formed} \\
    \mytoprule
    Future courses                                                     & \begin{tabular}[c]{@{}l@{}}52.4\%\\ (47.0\%, 57.8\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}97.2\%\\ (94.5\%, 99.9\%)\end{tabular} \\ \hline
    Group interaction                                              & \begin{tabular}[c]{@{}l@{}}56.6\%\\ (51.3\%, 61.9\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}95.8\%\\ (92.5\%, 99.1\%)\end{tabular} \\ \hline
     Group participation                                                     & \begin{tabular}[c]{@{}l@{}}62.3\%\\ (57.1\%, 67.5\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}95.1\%\\ (91.6\%, 98.6\%)\end{tabular} \\ \hline
    Comfort asking questions                                           & \begin{tabular}[c]{@{}l@{}}74.2\%\\ (69.6\%, 78.9\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}93.7\%\\ (89.7\%, 97.7\%)\end{tabular} \\ \hline
    Comfort sharing ideas                                              & \begin{tabular}[c]{@{}l@{}}78.4\%\\ (74.0\%, 82.9\%)\end{tabular}  & \begin{tabular}[c]{@{}l@{}}95.1\%\\ (91.7\%, 98.6\%)\end{tabular} \\ \hline
    \end{tabular}
    \caption{ Percentages (with confidence intervals) of students who reported positive responses to the five group quality indicators. First column: Students in software-matched groups. Second Column: Students in self-formed groups.}
    \label{fig:overall_props}
\end{figure}

==> sections/conclusion.tex <==
\section{Conclusion \& Future Work} \label{sec:conc_future_work}

The results presented in this paper stem from the Fall 2020 offering of EECS 16A at UC Berkeley. Since then, our research group has executed the matching process in numerous courses totalling over 3,000 students throughout the Spring 2021, Summer 2021, Fall 2021, and Spring 2022 semesters, and have had positive results based on preliminary looks at the data. A detailed analysis is yet to be conducted. Despite Fall 2021 and later semesters being in-person, we have found that study group formation continues to be in demand and well-used by courses. Student feedback has iteratively refined our process, and are experimenting with machine learning and reinforcement learning techniques to improve groups. We hope to soon release an open-source web-based privacy preserving version of our improved algorithm soon. 
